Domain-adaptive Video Deblurring via Test-time Blurring

Dynamic scene video deblurring aims to remove undesirable blurry artifacts captured during the exposure process. Although previous video deblurring methods have achieved impressive results, they suffer from significant performance drops due to the domain gap between training and testing videos, especially for those captured in real-world scenarios. To address this issue, we propose a domain adaptation scheme based on a blurring model to achieve test-time fine-tuning for deblurring models in unseen domains. Since blurred and sharp pairs are unavailable for fine-tuning during inference, our scheme can generate domain-adaptive training pairs to calibrate a deblurring model for the target domain. First, a Relative Sharpness Detection Module is proposed to identify relatively sharp regions from the blurry input images and regard them as pseudo-sharp images. Next, we utilize a blurring model to produce blurred images based on the pseudo-sharp images extracted during testing. To synthesize blurred images in compliance with the target data distribution, we propose a Domain-adaptive Blur Condition Generation Module to create domain-specific blur conditions for the blurring model. Finally, the generated pseudo-sharp and blurred pairs are used to fine-tune a deblurring model for better performance. Extensive experimental results demonstrate that our approach can significantly improve state-of-the-art video deblurring methods, providing performance gains of up to 7.54dB on various real-world video deblurring datasets. The source code is available at https://github.com/Jin-Ting-He/DADeblur.

==> Limitation.tex <==
\section{Limitation}
Our proposed method involves generating new domain-specific training data using pseudo-sharp images produced by RSDM and domain-specific blur conditions generated by DBCGM. However, it's important to note that if the input testing video is entirely very blurry without any relatively sharp regions, the effectiveness of RSDM will be limited. Table~\ref{Tab:Ablation_RSDM_threshold_specific_range} supports our conjecture, showing that performance drops when we deliberately use blurrier regions, specifically those within the 60\%-80\% range. Despite this, our results still outperform the baseline even when using blurrier regions for pseudo-sharp images. This is because the domain-specific blurred images generated through DBCGM and the reblurring model still enable the model to be stable when there are large domain gap between training data and testing data. Besides it also enable the model to learn deblurring information, achieving a certain level of deblurring effect.
